Experimental Demonstration Of Scanned Spin-Precession Microscopy

Progress in spintronics has been aided by characterization tools tailored to certain archetypical materials. New device structures and materials will require characterization tools that are material independent, provide sufficient resolution to image locally-varying spin properties and enable subsurface imaging. Here we report the demonstration of a novel spin-microscopy tool based on the variation of a global spin-precession signal in response to the localized magnetic field of a scanned probe. We map the local spin density in optically pumped GaAs from this spatially-averaged signal with a resolution of 5.5 microns. This methodology is also applicable to other spin properties and its resolution can be improved. It can extend spin microscopy to device structures not accessible by other techniques, such as buried interfaces and non-optically active materials, due to the universal nature of magnetic interactions between the spins and the probe.

==> fittingLineScans.tex <==
\section{Fitting the line scans}\label{sec:linescanFits}
The fits to the line scans shown in Fig.~3 of the main text were done using the convolution equation shown in Eqn.~1 of the main text\,(same as Eqn.~\ref{eq:ContinuumConv}). The various parameters for the fit were either measured independently or constrained by measured quantities. The $B_{1/2} = 1/\gamma\tau_s$ was obtained using Hanle measurement done far away from the $\mu P$. This Hanle data is shown in Fig.~\ref{fig:hanle}, along with the Lorenztian fitting done to obtain the halfwidth. The fitted $B_{1/2} = 111\,$G corresponds to a lifetime of $2.33$\,ns assuming a g-factor of -0.44 for GaAs. No diffusion\,($D = 0$) was assumed. A moment of $2\times10^{-9}$\, J/T  and a moment height of  $8\,\mu$m were used. These parameters provide a better fit\,(in terms of mean squared error) than $3\times10^{-9}$\, J/T  and $9\,\mu$m, which would have been nominally expected values given the particle radius\,($9\,\mu$m) as determined from SEM images. This may be due to the limitations of the simple single dipole model that we use for $\mu P$. The injection spot is assumed to be a Gaussian of $5\,\mu$m half-width, which is close to the the values obtained from fitting the camera image data to a 2D Gaussian. 
\begin{figure*}[htb]
\center{\includegraphics[scale = 0.75]{Hanles.pdf}}
\caption{Hanle curves measured far away from the $\mu P$ for the two spin density profiles $\rho_c$\,(red circles) and $\rho_u$\,(blue pluses).}	
	\label{fig:hanle}
\end{figure*}

==> imageExtraction2.tex <==
\section{Extracting the Spin Density}\label{sec:deconv}
\begin{figure*}[htb]
\center{\includegraphics[scale = 0.75]{TheoreticalDOIs.pdf}}
\caption{spin density $\rho_u$ obtained from deconvolution of $\Sigma_u$ and the theoretical PRFs shown in Fig.~3\textbf{a}\,(left hand panel) and Fig.3\textbf{b}\,(right hand panel) of the main text.}
	\label{fig:theoryDOI}
\end{figure*}

The PRFs presented in Fig.~4\textbf{a} and \textbf{b} were obtained by a Wiener deconvolution process,
\begin{equation}
H_B(R, B_t) = \Sigma_c({\bf r}_p, B_t) \circledast \rho({\bf r}_c).
\end{equation}
The deconvolution was implemented using Mathematica with a regularization parameter of 20. 

The PRFs presented in Fig.~4\textbf{c} and \textbf{d} were calculated using Eqns.~\ref{eq:HB}, \ref{eq:thetab1} and \ref{eq:dipole}, and the point dipole parameters used in sec.\ref{sec:linescanFits}. Fig.~\ref{fig:theoryDOI} presents the $\rho_u$ obtained by deconvolving using the theoretical PRFs in the main text from $\Sigma_u$, 
\begin{equation}
\rho({\bf r}_c) = \Sigma_c({\bf r}_p, B_t) \circledast H_B(R, B_t).
\end{equation}
These deconvolutions used a regularization parameter of 10.







==> measuredSignal.tex <==
\section{The measured signal}\label{sec:conv}
In our experiment the measured signal may be described by
\begin{equation}\label{eq:sigma}
\Sigma \propto \int_A S_z({\bf r})\,dx_sdy_s, 
\end{equation}
where $A$ represents the area of detection and can be assumed to extend to infinity. The magnetic field, $\bf B$, in our experiment is provided by the field from a micromagnetic probe\,($\mu P$), ${\bf B}_p$, and a spatially uniform field $B_t\hat{\bf x}$. Assuming the $\mu P$ to be a point dipole, the field experienced by the spins, at position ${\bf r}_s$ within the sample, is given by 
\begin{align}\label{eq:dipole}
{\bf B}({\bf R}) &= {\bf B}_p({\bf R}) + B_t\hat{x}\nonumber\\
&= \frac{\mu_0}{4\pi}\frac{3{\bf R}({\bf m}\cdot{\bf R})- {\bf m}R^2}{R^5}+ B_t\hat{\bf x}.
\end{align}
Here, ${\bf R} = {\bf r}_s - {\bf r}_p$ is the relative spatial vector between the position of the $\mu P$, ${\bf r}_p$, and the position of the spins within the sample; $\bf m$ is the moment of the $\mu P$ and $\mu_0$ is the permeability of free space.

Substituting Eqns.~\ref{eq:matrixsol} and \ref{eq:dipole} into Eqn.~\ref{eq:sigma}, we can write the measured signal as
\begin{align}
\Sigma({\bf r}_p) &\propto \int_\infty^\infty\int_\infty^\infty S_z({\bf r}_s, {\bf r}_p)\,dx_sdy_s \nonumber\\ 
&\propto  \int_\infty^\infty\int_\infty^\infty \left(\frac{1+B_z^{*2}({\bf R})}{1 + { B_x^*({\bf R})}^2+{ B_y^*({\bf R})}^2 + { B_z^*({\bf R})}^2}\right)\rho({\bf r}_s)\,dx_sdy_s \nonumber\\
&\propto H_B({\bf R}) \ast \rho({\bf r}_s).
\label{eq:ContinuumConv}
\end{align}
The $\star$ operator denotes a two-dimensional convolution integral and $H_B$ is the \emph{Precessional Response Function} ($PRF$), which may be written in the following manner to emphasize the physics at play
\begin{align}\label{eq:HB}
H_B({\bf R}) &= \frac{1+B_z^{*2}({\bf R})}{1 + {B_x^*({\bf R})}^2+{ B_y^*({\bf R})}^2 + {B_z^*({\bf R})}^2} \nonumber\\
&= \frac{1}{1 + \theta_B^2({\bf R})},
\end{align}
where the effective dephasing factor $\theta_B$ is given by
\begin{equation}
\theta_B^2( {\bf R} ) = \frac{\gamma^2B_\perp( {\bf R} )^2\tau_s^2}{1 + \gamma^2B_\|( {\bf R} )^2\tau_s^2},
\label{eq:thetab1}
\end{equation}
where $B_\| = \sqrt{B_x^2 + B_y^2}$ and $B_\perp = B_z$ refer to the parallel and perpendicular components of the total field $\bf B$, with respect to the injected spin direction $\hat{\bf z}$.
\begin{figure*}[htb]
\center{\includegraphics[scale = 0.75]{Linescan2.pdf}}
\caption{Background removal and normalization of spin signal $\Sigma$. All the data shown in the figure correspond to the line scan data shown in Fig.~3 of the main text\,($B_t = 0$, scan along $\hat{\bf x}$). Two lock-in signals $A-B$\,(blue dashed line, right axis) and A+B\,(green dashed line, right axis) are measured, where A and B correspond to the two photodiodes in the diode-bridge circuit.  These correspond to the difference and sum of the intensities of the two circularly polarized components of the PL. The spin density is then proportional to A-B/A+B\,(red solid line, left axis). The A-B and A+B channels can exhibit reflectivity changes\,(for e.g., the dip at $y_P~20\,\mu$m) as a function of the probe's position or due to the surface conditions of the sample. However, these are reasonably removed during the division process. Further evidence for the spurious reflectivity changes is seen in the spin-insensitive PL signal\,(black dashed line, right axis) collected by a separate photodiode. }
	\label{fig:measured signal}
\end{figure*}

==> opticalSetup.tex <==
\section{The optical set-up}\label{sec:optical set-up}
Spins are injected into the GaAs membrane using optical spin injection, which is a well established technique. The detection is based on measuring the circular polarization of the PL, which in turn is proportional to the spin polarization within the sample. The set-up used for optical pumping and the spin-PL measurements is shown in Fig.~\ref{fig:opticalSetup}. Also, provided in Table S1 is a detailed list of the various optical components used and their purpose. 

The Electro-Optic Modulator (EOM) allows us to modulate the polarization of light, and thus modulate the spin polarization within the sample, between $+\hat{\bf z}$ and $-\hat{\bf z}$, and enable lock-in measurements. The EOM modulates the 780\,nm pump between two linear polarization states. These are converted into the two circular states by the the Quarter Wave Plate (QWP). The circularly polarized laser light is focused on the sample\,(which sits inside an optical cryostat at a temperature of 17\,K) using an objective. A wire mesh is placed in the path of the pump beam to produce the spin density profile $\rho_u$\,(see main text). When producing different spin density profiles, the pump power was adjusted to keep the Hanle half-width far away from the $\mu P$ equal.
 
The circularly polarized light injects spins due to a combination of spin-orbit coupling and optical selection rules. The resulting PL due to the recombination of spin-polarized carriers is circularly polarzied. This PL\,(at the band edge of GaAs, ~819\,nm) is then collimated by the objective and converted back into the linear states by the QWP. The Wollaston prism splits the two orthogonal linear states; each of which is then collected by a separate photodiode that are part of a diode-bridge circuit. More details of how the photodiode signal is processed is presented in the next section.
 
The end of a multi-mode fiber is placed $\sim$1\,mm away from the sample (on the side opposite to laser injection, i.e. on the $\mu P$ side). The fiber is used for illuminating the sample with unpolarized broadband light\,(from a halogen lamp) to assist with camera imaging and tracking of the $\mu P$ during the measurements. The back illumination gives negligible spin signal for our lock-in measurements. 

Also, a variety of optical filters are used in various parts of the optical set-up to  remove unwanted light from reaching the photodiodes or the camera. Please see Table~S1 for more details.
\begin{figure*}[htb]
\center{\includegraphics[width = 0.95\linewidth]{experimentalsetupschematicfullrenderSmall.png}}
\caption{The optical set-up for the optical pumping and spin PL detection. Please see Table~S1 and sec.~\ref{sec:optical set-up} for more details of the various components.}
	\label{fig:opticalSetup}
\end{figure*}
 

==> scanningAndDataCollection.tex <==
\section{Scanning and data collection}\label{sec:data collection}
The data shown in Fig. 2\textbf{b},\textbf{c} and Fig.~4\textbf{a},\textbf{c} of the main text are obtained by scanning the objective\,(which in turn scans the pump beam relative to the sample) using motorized translation stages. The position of the $\mu P$ relative to the beam was tracked using a home built software solution. The Labview-based software uses the camera image and pattern recognition algorithms from National Instruments. This measured position in pixels of the camera image was converted into microns using a SEM image of the $\mu P$ as a calibration.

Fig.~\ref{fig:signal processingSetup} shows the instrumentation and hardware signal processing used for obtaining the spin signal from the photodiode voltages. The signals from the photo-diode bride allow us to compute the average steady state spin polarization within the sample, $\Sigma\propto \frac{V_{R} - V_{L}}{V_{R} + V_{L}}$, where the subscripts refer to right or left circular polarization of the PL. The difference signal, $V_{R} - V_{L}$, is the lockin signal due to the modulation of the polarization using the EOM. $V_{R} + V_{L}$ is measured as a different lock-in signal by modulating the power of the pump laser. The normalization by the sum of the two circular components removes spurious reflectivity changes in the signal, as seen in Fig.~\ref{fig:measured signal}.

The step size of the translation stages is somewhat variable. To allow for further data analysis, we have interpolated the 2D scan data\,(but not the line scan data) using Igor Pro software to have the signal on a uniform spatial grid. The data shown in the main text is the interpolated data. Further, all the data has been normalized such that $\Sigma$ far away from $\mu P$ at zero field and maximum field are taken to be 1 and 0 respectively. Also, for the line scans the position values were offset to bring the central peak to $x\,\mbox{or}\,y = 0$. 
\begin{figure*}[htb]
\center{\includegraphics[width = 0.95\linewidth]{signalprocessingschematicfullrenderSmall.png}}
\caption{Schematic of the signal processing done to obtain the measured signal. Please see Table~S1 and sec.~\ref{sec:data collection} for more details of the various components.}
	\label{fig:signal processingSetup}
\end{figure*}

==> spinDiffEqn.tex <==
\section{Spin dynamics in a non-magnetic material}\label{sec:formalism}
In a two-dimensional non-magnetic semiconductor, the spin density may be governed by the following equation of motion\cite{Furis:2007p479}
\begin{equation} 
\frac{\partial{\bf S}}{\partial t} = {\bf G} + D\nabla^2{\bf S} + \zeta({\bf E\cdot\nabla}){\bf S}
+ \gamma{\bf B}\times {\bf S}  - \frac{{\bf S}}{\tau_s},
\label{eq:diffeq}
\end{equation}
where all vector fields ($\bf S, G, E, B $) are, in general, functions of the spatial coordinate ${\bf r}_s = (x_s, y_s, 0)$ within the sample and time $t$. The spin density is given by $\bf S$; each component of this vector field gives the difference between spin ``up'' and ``down'' particle densities in that direction.  The first term on the R.H.S. of Eqn.~\ref{eq:diffeq}, ${\bf G}$, represents the rate at which spin density is externally injected and related to the intensity of the pump light. The second and third terms dictate the diffusion and drift of the spins respectively, where $D$ is the diffusion constant, $\bf E$ is the electric field, and $\zeta$ the electron\,(or hole) mobility. We assume no difference in diffusivity between opposite-spin carriers in any direction. The fourth term gives the precession of spin density around a net magnetic field ${\bf B}$, with $\gamma= g\mu_B/\hbar$ being the gyromagnetic ratio; where $g$ is the g-factor, $\mu_B$ is the Bohr magneton, and $\hbar$ the reduced Planck constant. The final term represents spin relaxation with a spin lifetime of $\tau_s$. 

We study the case in which ${\bf E} = {\bf 0}$, $\tau_s$ is spatially uniform, and ${\bf B}$ and ${\bf G}$ vary spatially but not in time.  We also consider an injection rate constrained to the $z$-axis, i.e. ${\bf G} = G_z \hat{z}$.  From a device point-of-view, one usually measures the steady-state solution of spin density $\textbf{S}(x,y,t \rightarrow \infty )$; in what follows we will only consider this solution. 

In the limit where diffusion is negligible, Eqn.~\ref{eq:diffeq} possesses a purely algebraic solution, which can be written more conveniently by introducing the following notation
\[{\cal B} = \left(\begin{array}{ccc}
0 	 & B_z^* 	& -B_y^* \\
-B_z^* & 0		& B_x^* \\
B_y^*  & -B_x ^*	& 0  \end{array} \right), \]
where we have applied a scaling to $\bf B$\,(and its vector components $B_x, B_y, B_z$), ${\bf B}^* = \gamma \tau_s {\bf B}$ . 

The steady state solution, $\partial{\bf S}/{\partial t} = 0$, for the case of $D = 0$ is then given by
\begin{equation}\label{case: D = 0}
{\bf S}({\bf r}) = [I - {\cal B}({\bf r}_s)]^{-1}\rho({\bf r}_s)\\
\end{equation}
where, $\rho({\bf r}_s) = G_z({\bf r}_s)\tau_s$. It should be noted that $\bm \rho$ is the steady state spin density in the absence of any magnetic field and is the quantity that we are interested in measuring in this experiment from a signal that is averaged in $\bf r$. 

Seen in the above equation is that fact that the absence of both drift and diffusion eliminates all coupling between neighboring positions (which in general are coupled due to derivative operators).  Thus, in this particular limit, the steady-state solution is determined algebraically by the magnetic field values at a given position, and does not need to be solved using the full differential equation. The solutions, based on Eqn.~\ref{case: D = 0}, for the various vector components of $\bf S({\bf r}_s)$ are determined by $B$ and $\rho$ only at that ${\bf r}_s$; they are given by,
\begin{subequations} \label{eq:matrixsol}
\begin{align}
S_x &=  \frac{B_x^*B_z^* - B_y^*}{1 + { B_x^*}^2+{ B_y^*}^2 + {B_z^*}^2}\rho\\
S_y &=  \frac{B_y^*B_z^* + B_x^*}{1 + { B_x^*}^2+{ B_y^*}^2 + { B_z^*}^2}\rho\\
S_z &=  \frac{1+B_z^{*2}}{1 + { B_x^*}^2+{ B_y^*}^2 + { B_z^*}^2}\rho,
\end{align}
\end{subequations}




==> table1.tex <==
\begin{table}[htb]
\begin{center}
\begin{tabular}{|c|r@{\extracolsep{0pt}.}l|c|}
\hline 
S.no & \multicolumn{2}{c|}{Description} & Comments\tabularnewline
\hline 
\hline 
A & \multicolumn{2}{c|}{GaAs sample} & see section I for more details\tabularnewline
\hline 
B & \multicolumn{2}{c|}{Electromagnet} & Power supply controlled via DAQ card \tabularnewline
\hline 
C & \multicolumn{2}{c|}{Optical crystat} & Operated at 17K\tabularnewline
\hline 
D & \multicolumn{2}{c|}{Objective lens} & plan fluor 10X\tabularnewline
\hline 
E & \multicolumn{2}{c|}{Quarter-wave plate} & \tabularnewline
\hline 
F & \multicolumn{2}{c|}{Dichroic mirror} & Reflects pump towards the sample, but attentuates it during transmission \tabularnewline
\hline 
G & \multicolumn{2}{c|}{Notch Filter} & For 780 nm\tabularnewline
\hline 
H & \multicolumn{2}{c|}{Cube beam splitter} & Non-polarizing\tabularnewline
\hline 
I & \multicolumn{2}{c|}{Focusing lens} & f = 100 mm\tabularnewline
\hline 
J & \multicolumn{2}{c|}{Wollaston prism} & Separates the two linear polarization components\tabularnewline
\hline 
K & \multicolumn{2}{c|}{Bandpass filter} & Centered at 820 nm, 10 nm width\tabularnewline
\hline 
L & \multicolumn{2}{c|}{Photodiode bridge} & The difference channel is amplified by a factor of 100000 \tabularnewline
\hline 
M & \multicolumn{2}{c|}{focusing lens} & f = 200 mm\tabularnewline
\hline 
N & \multicolumn{2}{c|}{Cube beam splitter} & \tabularnewline
\hline 
O & \multicolumn{2}{c|}{Long pass filter} & cut off at 850nm\tabularnewline
\hline 
P & \multicolumn{2}{c|}{CMOS camera} & \tabularnewline
\hline 
Q & \multicolumn{2}{c|}{Photodiode} & To measure spin-insensitive DC level of the PL\tabularnewline
\hline 
R & \multicolumn{2}{c|}{Wire mesh} & \tabularnewline
\hline 
S & \multicolumn{2}{c|}{Electro-optic modulator} & Modulated polarization of light \tabularnewline
\hline 
T & \multicolumn{2}{c|}{Polarizer} & transmits vertical polarization, as needed for the EOM operation\tabularnewline
\hline 
U & \multicolumn{2}{c|}{Polarizer} & Allows for fine control of pump power\tabularnewline
\hline 
V & \multicolumn{2}{c|}{ND filters} & \tabularnewline
\hline 
W & \multicolumn{2}{c|}{Pump laser} & 780 nm, stable laser source, intensity modulated\tabularnewline
\hline 
X & \multicolumn{2}{c|}{Function generator} & used to provide modulation signal for EOM, square, $f_{mod} \sim 73$\,Hz\tabularnewline
\hline 
Y & \multicolumn{2}{c|}{Voltage preamplifier} & Amplifies the A-B channel of the dide bridge, Gain of 200\tabularnewline
\hline 
Z & \multicolumn{2}{c|}{Voltage preamplifier} & Amplifies the B channel of the dide bridge, Gain of -1000\tabularnewline
\hline 
AA & \multicolumn{2}{c|}{Voltage preamplifier} & Amplifies the A channel of the diode bridge, Gain of 1000\tabularnewline
\hline 
AB & \multicolumn{2}{c|}{Lock-in amplifier} & Demodulates the pump power modulation, typical time const. 200-500ms\tabularnewline
\hline 
AC & \multicolumn{2}{c|}{Lock-in amplifier} & Demodulates the EOM modulation, typical time const. 200-500ms\tabularnewline
\hline 
AD & \multicolumn{2}{c|}{Function generator} & used to provide modulation signal for pump intensity, square, $f_{mod} \sim 1100$\,Hz\tabularnewline
\hline 
AE & \multicolumn{2}{c|}{Computer} & Controls the instruments and performs data acq., thru GPIB and DAQ
card\tabularnewline
\hline 
\end{tabular}
\end{center}
\caption{A list of the various optical components and electronic instruments used in the experiment. The s.no correspond to the letters in Fig.~\ref{fig:opticalSetup} and \ref{fig:signal processingSetup}.}
\label{table:1}
\end{table}
